Preference Leakage: A Contamination Problem in LLM-as-a-judge

Large Language Models (LLMs) as judges and LLM-based data synthesis have emerged as two fundamental LLM-driven data annotation methods in model development. While their combination significantly enhances the efficiency of model training and evaluation, little attention has been given to the potential contamination brought by this new model development paradigm. In this work, we expose preference leakage, a contamination problem in LLM-as-a-judge caused by the relatedness between the synthetic data generators and LLM-based evaluators. To study this issue, we first define three common relatednesses between the data generator LLM and the judge LLM: being the same model, having an inheritance relationship, and belonging to the same model family. Through extensive experiments, we empirically confirm the bias of judges towards their related student models caused by preference leakage across multiple LLM baselines and benchmarks. Further analysis suggests that preference leakage is a pervasive and real-world problem that is harder to detect compared to previously identified biases in LLM-as-a-judge scenarios. All of these findings imply that preference leakage is a widespread and challenging problem in the area of LLM-as-a-judge. We release all codes and data at: https://github.com/David-Li0406/Preference-Leakage.

==> iclr2026/Preference_Leakage.tex <==
\subsection{LLMs as Oracles: A New Avenue for Contamination}

With the advent of LLMs, these models are increasingly employed as ``oracles'' in various scenarios: for both synthetic data generation ($M_G$) and employed as evaluators ($M_J$) to automate the assessment. While these approaches enhance scalability and efficiency, they also introduce potential risks. Specifically, if the LLM used for data generation ($M_G$) and the LLM used for evaluation ($M_J$) are not independent, a new contamination—preference leakage—can emerge, biasing evaluation outcomes.

\subsection{Defining Preference Leakage in LLM-based Evaluation}

Formally, to define preference leakage, we consider the following entities in models development:

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt,parsep=1pt]
    \item \textbf{Data Generator LLM, $M_G$}, defining a conditional distribution $P_{M_G}(y|x)$ for generating an output $y$ given a prompt $x$, forming the synthetic dataset $D_{syn}$ for student LLMs training.
    \item \textbf{Student LLM, $M_S$}, trained on data generated by $M_G$, producing an output distribution $P_{M_S}(y|x)$.
    \item \textbf{Judge LLM, $M_J$}, providing a scoring function $S_{M_J}(y|x)$ that assesses output $y$ for prompt $x$.
\end{itemize}

Preference leakage occurs when the evaluation score assigned by $M_J$ to $M_S$'s outputs is inflated due to an underlying relatedness between $M_G$ and $M_J$. This implies that $M_J$ may favor outputs from $M_S$ not solely based on their intrinsic quality, but because they exhibit spurious features (e.g., style, format, wording) inherited from $M_G$, to which $M_J$ is predisposed due to this relatedness:

\begin{equation}
\label{eq:pref_leakage}
    E_{x, y_S \sim P_{M_S}}[S_{M_J}(y_S|x) | M_G \sim_{rel} M_J] > E_{x, y_S \sim P_{M_S}}[S_{M_{J'}}(y_S|x) | M_G \not\sim_{rel} M_{J'}],
\end{equation}

where $y_S$ are outputs from $M_S$. The relation $M_G \sim_{rel} M_J$ denotes that judge $M_J$ is related to $M_G$, while $M_G \not\sim_{rel} M_{J'}$ denotes that an alternative judge $M_{J'}$ is not related to $M_G$ and possess comparable intrinsic quality assessment capabilities to $M_J$. The expectation is taken over the input distribution $\mathcal{X}$ and the trained Student LLM's output distribution $P_{M_S}$.

\subsection{Type of LLM ``Relatedness''}

The condition $M_G \sim_{rel} M_J$ in Equation~\ref{eq:pref_leakage} encapsulates several ways the Data Generator LLM and Judge LLM can be interconnected. We identify three common types in the real world:

\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt,parsep=1pt]
    \item \textbf{Being the Same Model:} The most direct form of relatedness occurs when the Data Generator LLM and the Judge LLM are the exact same model instance:
    \begin{equation}
        M_G \equiv M_J.
    \end{equation}
    In this scenario, the inherent preferences in the model that shape its generative distribution $P_{M_G}(y|x)$ are precisely the same as those guiding its evaluation via the scoring function $S_{M_G}(y|x)$.

    \item \textbf{Inheritance Relationship:} One model's development is directly based on another, either by fine-tuning the existing model or by training a new model on the other's outputs, for instance:
    \begin{equation}
         M_J \leftarrow \text{FineTune}(M_G, D_{train}) \quad \text{or} \quad M_J \leftarrow \text{FineTune}(M_{base}, D_{syn_G}),
    \end{equation}
    where $D_{train}$ represents general training data used to adapt $M_G$ into $M_J$, $M_{base}$ is a base model, and $D_{syn_G}$ denotes synthetic data generated by $M_G$. This type of relationship is bidirectional; $M_G$ can similarly inherit from $M_J$ through analogous processes. In such cases, the descendant model is likely to internalize and thus favor the preferences, styles, or biases of its progenitor.

    \item \textbf{Within the Same Model Family:} The Data Generator LLM $M_G$ and Judge LLM $M_J$ belong to the same model family (e.g., different versions or sizes of GPT). Models within such a family typically share a common architectural blueprint ($A_X$) and are often developed from foundational models pre-trained on substantially overlapping datasets ($D_X$).
    This shared foundation ($A_X, D_X$) would lead to correlated preferences and systemic biases characteristic of the common origin:
    \begin{equation}
        M_k \in \text{Family}(A_X, D_X) \quad \text{for } k \in \{G, J\}.
    \end{equation}
\end{itemize}

% Due to these forms of relatedness, the preferences of the Judge LLM $M_J$ (e.g., regarding format, style, and wording) can be inadvertently aligned with those of the Data Generator LLM $M_G$. This alignment can cause the trained Student LLM $M_S$, trained on data from $M_G$, to receive inflated scores from $M_J$, not necessarily due to superior generalizable performance but due to echoing $M_G$'s leaked preferences.

==> iclr2026/prompt_category_dimension.tex <==
\begin{tcolorbox}[breakable, title=Judgment Dimension Categorization Prompt, label=test]
\small
\ttfamily
Given a pairwise comparison judgment made by an AI, please categorize each considered aspect in the rationale to one of the following categories:

\vspace{4mm}
\{
    
    \vspace{2mm}
    "Factuality": "Whether the information provided in the response is accurate, based on reliable facts and data.",

    \vspace{2mm}
    "User Satisfaction": "Whether the response meets the user's question and needs, and provides a comprehensive and appropriate answer to the question.",

    \vspace{2mm}
    "Logical Coherence": "Whether the response maintains overall consistency and logical coherence between different sections, avoiding self-contradiction.",

    \vspace{2mm}
    "Richness": "Whether the response includes rich info, depth, context, diversity, detailed explanations and examples to meet user needs and provide a comprehensive understanding.",

    \vspace{2mm}
    "Creativity": "Whether the response is innovative or unique, providing novel insights or solutions.",

    \vspace{2mm}
    "Fairness and Responsibility": "Whether the advice or information provided in the response is feasible, carries acertain degree of responsibility, and considers potential risks and consequences.",

    \vspace{2mm}
    "Completeness": "Whether the response provides sufficient information and details to meet the user's needs, and whether it avoids omitting important aspects.",

    \vspace{2mm}
    "Clarity": "Whether the response is clear and understandable, and whether it uses concise language and structure so that the user can easily understand it.",

    \vspace{2mm}
    "Others": "Other aspects which is not listed above."

\}

\vspace{4mm}
\#\# Judgment: [JUDGMENT]

\vspace{4mm}
Please output the generated content in a json format, for example:
\{
"Factuality": // list, all aspects that belong to this category, such as ["correctness", "mistakes"]
...
\}

\vspace{4mm}
Formatted the abovementioned schema and categorize aspects in the judgment:


\end{tcolorbox}
\label{}

==> iclr2026/prompt_pairwise_feedback.tex <==
\begin{tcolorbox}[breakable, title=Pairwise Feedback Prompt, label=More Cases]
\small
\ttfamily

Please act as an impartial judge and evaluate the quality of the responses provided by two AI assistants to the user question displayed below. Your evaluation should consider correctness and helpfulness. You will be given assistant A's answer, and assistant B's answer. Your job is to evaluate which assistant's answer is better. You should independently solve the user question step-by-step first. Then compare both assistants' answers with your answer. Identify and correct any mistakes. Avoid any position biases and ensure that the order in which the responses were presented does not influence your decision. Do not allow the length of the responses to influence your evaluation. Do not favor certain names of the assistants. Be as objective as possible. After providing your explanation, output your final verdict by strictly following this format: "[[A]]" if 
assistant A is better, "[[B]]" if assistant B is better.

\vspace{4mm}
\#\# Instruction: {}

\vspace{4mm}
[The Start of Assistant A's Answer]

[RESPONSE A]

[The End of Assistant A's Answer]

\vspace{4mm}
[The Start of Assistant B's Answer]

[RESPONSE B]

[The End of Assistant B's Answer]

\vspace{4mm}
Please output the generated content in a json format, for example:
\{
"reason": // string, reasons behind the chosen preferred answer
"prefered answer": // string, the prefered answer you selected, [[A]] or [[B]]
\}

\vspace{4mm}
Formatted the abovementioned schema and produce the reason and preferred answer:


\end{tcolorbox}
\label{}

==> iclr2026/prompt_recognition.tex <==
\begin{tcolorbox}[breakable, title=Pointwise Recognition Prompt, label=More Cases]
\small
\ttfamily
Given an instruction and a response, your task is to judge whether this response is generated by a model that is trained on a synthetic dataset you produced (your student model).

\vspace{4mm}
\#\# Instruction: [INSTRUCTION]

\vspace{4mm}
\#\# Response: [Response]

\vspace{4mm}
Please output the generated content in a json format, for example:
{{
"reason": // string, reasons behind the judgment
"judgment": // string, whether the answer is generated by your student model, choose from yes or no
}}

\vspace{4mm}
Formatted the abovementioned schema and produce the reason and judgment:


\end{tcolorbox}
\label{}

==> iclr2026/prompt_recognition_pairwise.tex <==
\begin{tcolorbox}[breakable, title=Pairwise Recognition Prompt, label=More Cases]
\small
\ttfamily
Given an instruction and two responses, your task is to judge which response is generated by a model that is trained on a synthetic dataset you produced (your student model).

\vspace{4mm}
\#\# Instruction: [INSTRUCTION]

\vspace{4mm}
\#\# Response1: [Response 1]

\vspace{4mm}
\#\# Response2: [Response 2]

\vspace{4mm}
Please output the generated content in a json format, for example:
{{
"reason": // string, reasons behind the judgment
"judgment": // int, 1 or 2, means response1 or response2 is from your student model 
}}

\vspace{4mm}
Formatted the abovementioned schema and produce the reason and judgment:


\end{tcolorbox}
\label{}
